Towards Event Extraction from Speech with Contextual Clues

While text-based event extraction has been an active research area and has seen successful application in many domains, extracting semantic events from speech directly is an under-explored problem. In this paper, we introduce the Speech Event Extraction (SpeechEE) task and construct three synthetic training sets and one human-spoken test set. Compared to event extraction from text, SpeechEE poses greater challenges mainly due to complex speech signals that are continuous and have no word boundaries. Additionally, unlike perceptible sound events, semantic events are more subtle and require a deeper understanding. To tackle these challenges, we introduce a sequence-to-structure generation paradigm that can produce events from speech signals in an end-to-end manner, together with a conditioned generation method that utilizes speech recognition transcripts as the contextual clue. We further propose to represent events with a flat format to make outputs more natural language-like. Our experimental results show that our method brings significant improvements on all datasets, achieving a maximum F1 gain of 10.7%. The code and datasets are released on https://github.com/jodie-kang/SpeechEE.

==> Submission/CoverLetter.tex <==
% 3 phases
% 第一段: 声明原创且未同时投稿其他杂志
% 第二段：陈述文章创新点
% 第三段：陈述文章的贡献，重要意义，以及为什么适合这个杂志

% I want you to act as an academic journal editor. I will provide you with the title and abstract of my manuscript. You need to write a format cover letter for submitting the manuscript to the IEEE/ACM Transactions on Audio, Speech, and Language Processing journal. This journal is dedicated to innovative theory and methods for processing signals representing audio, speech and language, and their applications. This includes analysis, synthesis, enhancement, transformation, classification, and interpretation of such signals as well as the design, development, and evaluation of associated signal processing systems.
% "Task": You should state that the manuscript is not considered for publication in any other journal. Briefly introduce the merit of the manuscript and provide a summary to point out the importance of the results for a scientific audience. The title and abstract are as follows: 
% "Title": Towards Event Extraction from Speech with Contextual Clues
% "Abstract": While text-based event extraction has been an active research area and has seen successful application in many domains, extracting semantic events from speech directly is an under-explored problem. In this paper, we introduce the Speech Event Extraction (SpeechEE) task and construct three synthetic training sets and one human-spoken test set. Compared to event extraction from text, SpeechEE poses greater challenges mainly due to complex speech signals that are continuous and have no word boundaries. Additionally, unlike perceptible sound events, semantic events are more subtle and require a deeper understanding. To tackle these challenges, we introduce a sequence-to-structure generation paradigm that can produce events from speech signals in an end-to-end manner, together with a conditioned generation method that utilizes speech recognition transcripts as the contextual clue. We further propose to represent events with a flat format to make outputs more natural language-like. Our experimental results show that our method brings significant improvements on all datasets, achieving a maximum F1 gain of 10.7\%.

Dear Editor,

I hope this letter finds you well. I am submitting our manuscript titled "Towards Event Extraction from Speech with Contextual Clues" for consideration in the TASLP. This manuscript is an original work and has not been concurrently submitted to any other journals.

The main innovation of our manuscript lies in addressing the under-explored problem of extracting semantic events directly from speech signals. While text-based event extraction has been widely researched and applied, extending this capability to speech introduces unique challenges, given the continuous and boundary-less nature of speech signals. We introduce the Speech Event Extraction (SpeechEE) task, offering a new perspective on event extraction that requires a more nuanced understanding of subtle semantic events within speech.

Our contribution to the field is three-fold. Firstly, we introduce a novel task, present benchmarks, and construct baselines. Secondly, we propose a sequence-to-structure generation paradigm that allows for end-to-end event extraction from speech signals. This paradigm is particularly designed to handle the complexities introduced by the continuous nature of speech. Thirdly, we introduce a conditioned generation method that utilizes speech recognition transcripts as contextual clues, aiding the model in overcoming the challenges of semantic event extraction.

The significance of our work extends beyond addressing the technical challenges associated with SpeechEE. We believe our approach has the potential to open new avenues for real-world applications, where the direct extraction of semantic events from spoken language can provide richer and more contextually relevant information.

We believe that our manuscript aligns well with the scope of the TASLP. The proposed methodology and the achieved experimental results demonstrate the efficacy of our approach. We hope that our work will contribute to the ongoing discourse on innovative theories and methods for processing signals representing audio, speech, and language.

Thank you for considering our manuscript for review. We look forward to the opportunity for our work to be reviewed by the distinguished panel of experts at the TASLP.

Sincerely,

Kang Jingqi
Towards Event Extraction from Speech with Contextual Clues
Southeast University

